RECAST: Approaching experimental accuracy in theoretical calculations of crystal structures

Many physical properties of materials are highly sensitive to their crystal structures. However, density-functional theory (DFT) yields systematic errors in cell volumes, shapes and atomic positions - a trait that is inherited by machine-learned interatomic potentials (MLIPs) trained on DFT data. Here we introduce RECAST (refinement of calculated structures), an equivariant method that learns to transform calculated structures towards their experimental counterparts. Trained on 18,056 calculated-experimental structure pairs, it predicts how each interatomic distance should change. A global structural fit incorporates these corrections as an effective energy contribution balanced against crystal stiffness, concentrating deformation in softer modes. RECAST lowers the held-out mean volume error from 4.12% to 0.85% and removes a third of the cell-shape and half of the bond-length error. Training it on universal-MLIP relaxations yields comparable gains, enabling their structures to be corrected towards experiment on the fly. Calculated structures can thus approach experimental accuracy without measurement.

==> tables/shape_numbers.tex <==
\newcommand{\shpN}{7{,}712}
\newcommand{\shpTailN}{433}
\newcommand{\shpTailShare}{27}
\newcommand{\shpTailFin}{3.27}
\newcommand{\shpTailPBE}{4.62}
\newcommand{\shpCos}{0.99}
\newcommand{\shpRatio}{0.34}
\newcommand{\shpNegRows}{31}
\newcommand{\shpNegErr}{33}
\newcommand{\shpNegGain}{25}
\newcommand{\shpOtherGain}{31}
\newcommand{\shpNLn}{2{,}000}
\newcommand{\shpNLconv}{99}
\newcommand{\shpNLsprTailLin}{3.29}
\newcommand{\shpNLsprTailNl}{3.96}
\newcommand{\shpNLsprp}{0.47}
\newcommand{\shpNLsprt}{0.76}
\newcommand{\shpNLcellp}{0.44}
\newcommand{\shpNLcellt}{0.81}
\newcommand{\shpNLalong}{7.6}
\newcommand{\shpNLdvol}{5.5}
\newcommand{\shpStN}{196}
\newcommand{\shpStStruct}{134}
\newcommand{\shpStNoMin}{188}
\newcommand{\shpStNoMinNoD}{119}
\newcommand{\shpStNoMinMol}{84}
\newcommand{\shpStNoMinD}{69}
\newcommand{\shpStSlow}{8}
\newcommand{\shpStSlowStruct}{8}
\newcommand{\shpUndefN}{144}
\newcommand{\shpUndefDrop}{0.02}


==> tables/si_tables.tex <==
\newcommand{\tabpartcell}{42 & 1{,}794 & 4.10 & 0.86 & 0.93 & 0.65 & 0.67 & 1.42 & 0.43 & 0.11 & 0.07\\
43 & 1{,}794 & 4.10 & 0.89 & 0.93 & 0.64 & 0.68 & 1.43 & 0.44 & 0.11 & 0.08\\
44 & 1{,}792 & 4.16 & 0.86 & 0.94 & 0.65 & 0.68 & 1.45 & 0.43 & 0.11 & 0.07\\
45 & 1{,}796 & 4.10 & 0.83 & 0.93 & 0.64 & 0.66 & 1.41 & 0.42 & 0.11 & 0.08\\
46 & 1{,}787 & 4.21 & 0.87 & 0.96 & 0.65 & 0.69 & 1.45 & 0.43 & 0.11 & 0.08\\
47 & 1{,}795 & 4.05 & 0.79 & 0.92 & 0.65 & 0.67 & 1.41 & 0.41 & 0.11 & 0.08\\
48 & 1{,}796 & 4.13 & 0.82 & 0.94 & 0.64 & 0.66 & 1.43 & 0.42 & 0.11 & 0.08\\
49 & 1{,}797 & 4.12 & 0.86 & 0.96 & 0.65 & 0.68 & 1.44 & 0.43 & 0.11 & 0.08\\
50 & 1{,}794 & 4.12 & 0.86 & 0.94 & 0.65 & 0.67 & 1.42 & 0.42 & 0.11 & 0.08\\
51 & 1{,}792 & 4.13 & 0.84 & 0.89 & 0.62 & 0.65 & 1.42 & 0.41 & 0.11 & 0.08\\}
\newcommand{\tabpartatoms}{42 & 1.64 & 0.96 & 0.74 & 0.85 & 0.043 & 0.035 & 0.89 & 0.77\\
43 & 1.63 & 0.94 & 0.75 & 0.86 & 0.041 & 0.035 & 0.88 & 0.77\\
44 & 1.66 & 0.98 & 0.76 & 0.87 & 0.042 & 0.035 & 0.90 & 0.76\\
45 & 1.66 & 0.97 & 0.75 & 0.86 & 0.043 & 0.036 & 0.93 & 0.80\\
46 & 1.67 & 0.97 & 0.76 & 0.87 & 0.043 & 0.036 & 0.91 & 0.79\\
47 & 1.62 & 0.96 & 0.74 & 0.84 & 0.043 & 0.036 & 0.91 & 0.77\\
48 & 1.60 & 0.93 & 0.71 & 0.82 & 0.041 & 0.035 & 0.88 & 0.76\\
49 & 1.70 & 1.01 & 0.79 & 0.90 & 0.045 & 0.037 & 0.98 & 0.84\\
50 & 1.64 & 0.97 & 0.75 & 0.86 & 0.042 & 0.035 & 0.89 & 0.76\\
51 & 1.63 & 0.94 & 0.74 & 0.85 & 0.042 & 0.035 & 0.89 & 0.77\\}
\newcommand{\tabstrata}{$s_{\rm DFT}<1\%$ & 12{,}532 & 0.35 & 0.31 & 0.31 & 0.30 & 3.78 & 0.75 & 0.73 & 0.72 & 1.50 & 0.74\\
$1\leq s_{\rm DFT}<3\%$ & 4{,}308 & 1.68 & 1.08 & 1.04 & 1.03 & 4.81 & 1.01 & 0.96 & 0.95 & 1.84 & 0.98\\
$s_{\rm DFT}\geq3\%$ & 1{,}097 & 4.60 & 3.19 & 3.02 & 3.02 & 5.38 & 1.96 & 1.91 & 1.89 & 2.57 & 1.73\\
0D & 832 & 1.20 & 0.98 & 0.99 & 0.98 & 4.83 & 1.42 & 1.48 & 1.47 & 2.13 & 1.04\\
1D & 283 & 1.84 & 1.19 & 1.18 & 1.18 & 5.70 & 1.09 & 1.10 & 1.10 & 2.01 & 0.99\\
2D & 747 & 2.01 & 1.31 & 1.25 & 1.25 & 5.17 & 1.32 & 1.27 & 1.25 & 1.64 & 0.86\\
3D & 16{,}075 & 0.85 & 0.62 & 0.59 & 0.59 & 4.01 & 0.83 & 0.80 & 0.79 & 1.62 & 0.84\\
same space group & 17{,}511 & 0.93 & 0.67 & 0.65 & 0.64 & 4.13 & 0.88 & 0.86 & 0.85 & 1.64 & 0.85\\
space group differs & 426 & 1.01 & 0.73 & 0.72 & 0.71 & 3.93 & 1.03 & 0.98 & 0.98 & 1.72 & 1.01\\
high-pressure phase & 446 & 0.73 & 0.55 & 0.53 & 0.53 & 4.09 & 1.29 & 1.26 & 1.24 & 1.45 & 0.71\\
high- or low-$T$ phase & 507 & 1.00 & 0.74 & 0.73 & 0.73 & 4.13 & 1.22 & 1.21 & 1.21 & 1.79 & 1.16\\}
\newcommand{\tabsize}{1--4 & 1{,}507 & 3.29 & 1.39 & 0.50 & 0.43 & 1.21 & 0.61\\
5--8 & 2{,}117 & 3.22 & 0.95 & 1.05 & 0.74 & 1.46 & 0.83\\
9--16 & 3{,}133 & 3.93 & 0.83 & 1.07 & 0.70 & 1.65 & 0.91\\
17--32 & 4{,}339 & 4.31 & 0.77 & 1.02 & 0.70 & 1.69 & 0.87\\
33--64 & 4{,}298 & 4.61 & 0.74 & 0.95 & 0.65 & 1.75 & 0.86\\
65--200 & 2{,}543 & 4.47 & 0.78 & 0.74 & 0.52 & 1.78 & 0.91\\}
\newcommand{\tabcs}{1{,}132 & 4{,}419 & 4{,}581 & 2{,}417 & 1{,}468 & 1{,}517 & 2{,}522}


==> tables/si_tables_extra.tex <==
\newcommand{\tabstratablocks}{\multicolumn{12}{@{}l}{\emph{DFT shape error}}\\
$s_{\rm DFT}<1\%$ & 12{,}532 & 0.35 & 0.31 & 0.31 & 0.30 & 3.78 & 0.75 & 0.73 & 0.72 & 1.50 & 0.74\\
$1\leq s_{\rm DFT}<3\%$ & 4{,}308 & 1.68 & 1.08 & 1.04 & 1.03 & 4.81 & 1.01 & 0.96 & 0.95 & 1.84 & 0.98\\
$s_{\rm DFT}\geq3\%$ & 1{,}097 & 4.60 & 3.19 & 3.02 & 3.02 & 5.38 & 1.96 & 1.91 & 1.89 & 2.57 & 1.73\\
\addlinespace
\multicolumn{12}{@{}l}{\emph{Dimensionality of the bonded network}}\\
0D & 832 & 1.20 & 0.98 & 0.99 & 0.98 & 4.83 & 1.42 & 1.48 & 1.47 & 2.13 & 1.04\\
1D & 283 & 1.84 & 1.19 & 1.18 & 1.18 & 5.70 & 1.09 & 1.10 & 1.10 & 2.01 & 0.99\\
2D & 747 & 2.01 & 1.31 & 1.25 & 1.25 & 5.17 & 1.32 & 1.27 & 1.25 & 1.64 & 0.86\\
3D & 16{,}075 & 0.85 & 0.62 & 0.59 & 0.59 & 4.01 & 0.83 & 0.80 & 0.79 & 1.62 & 0.84\\
\addlinespace
\multicolumn{12}{@{}l}{\emph{Space group}}\\
same space group & 17{,}511 & 0.93 & 0.67 & 0.65 & 0.64 & 4.13 & 0.88 & 0.86 & 0.85 & 1.64 & 0.85\\
space group differs & 426 & 1.01 & 0.73 & 0.72 & 0.71 & 3.93 & 1.03 & 0.98 & 0.98 & 1.72 & 1.01\\
\addlinespace
\multicolumn{12}{@{}l}{\emph{Phase}}\\
high-pressure phase & 446 & 0.73 & 0.55 & 0.53 & 0.53 & 4.09 & 1.29 & 1.26 & 1.24 & 1.45 & 0.71\\
high- or low-$T$ phase & 507 & 1.00 & 0.74 & 0.73 & 0.73 & 4.13 & 1.22 & 1.21 & 1.21 & 1.79 & 1.16\\
\addlinespace
\multicolumn{12}{@{}l}{\emph{Functional}}\\
DFT & 14{,}701 & 0.91 & 0.66 & 0.64 & 0.64 & 3.96 & 0.90 & 0.88 & 0.87 & 1.57 & 0.83\\
DFT+$U$ & 3{,}236 & 1.02 & 0.71 & 0.68 & 0.67 & 4.87 & 0.81 & 0.77 & 0.76 & 1.96 & 0.98\\
\addlinespace
\multicolumn{12}{@{}l}{\emph{Atoms in the cell}}\\
1--4 & 1{,}507 & 0.50 & 0.40 & 0.44 & 0.43 & 3.29 & 1.40 & 1.42 & 1.39 & 1.21 & 0.61\\
5--8 & 2{,}117 & 1.05 & 0.78 & 0.75 & 0.74 & 3.22 & 0.97 & 0.96 & 0.95 & 1.46 & 0.83\\
9--16 & 3{,}133 & 1.07 & 0.75 & 0.71 & 0.70 & 3.93 & 0.88 & 0.84 & 0.83 & 1.65 & 0.91\\
17--32 & 4{,}339 & 1.02 & 0.73 & 0.70 & 0.70 & 4.31 & 0.81 & 0.78 & 0.77 & 1.69 & 0.87\\
33--64 & 4{,}298 & 0.95 & 0.67 & 0.65 & 0.65 & 4.61 & 0.79 & 0.75 & 0.74 & 1.75 & 0.86\\
65--200 & 2{,}543 & 0.74 & 0.54 & 0.53 & 0.52 & 4.47 & 0.82 & 0.78 & 0.78 & 1.78 & 0.91\\}
\newcommand{\tabsimple}{constant correction & 17{,}937 & 4.12 & 2.08 & 0.85 & 0.93 & 0.93 & 0.64\\
hydrostatic pressure & 16{,}354 & 4.02 & 0.00 & 0.79 & 0.87 & 1.07 & 0.60\\
relaxation with D3 & 17{,}712 & 4.11 & 2.92 & 0.84 & 0.93 & 1.28 & 0.64\\
relaxation without D3 & 17{,}570 & 4.09 & 5.16 & 0.83 & 0.93 & 1.63 & 0.64\\}
\newcommand{\tabrefAsi}{all five, three initializations each (the correction) & 15 & 0.85 & 0.64 & 0.42 & 0.08 & 0.86\\
all five, one initialization each & 5 & 0.86 & 0.65 & 0.43 & 0.08 & 0.86\\
direct strain head, three initializations & 3 & 0.92 & 0.71 & 0.46 & 0.09 & 0.87\\
direct strain head, five initializations & 5 & 0.91 & 0.70 & 0.46 & 0.09 & 0.87\\
estimator 5, three initializations & 3 & 0.88 & 0.65 & 0.43 & 0.08 & 0.86\\
estimator 5, five initializations & 5 & 0.87 & 0.65 & 0.43 & 0.08 & 0.86\\
estimators 1--3, three initializations each & 9 & 0.86 & 0.66 & 0.43 & 0.08 & 0.86\\
estimators 4--5, three initializations each & 6 & 0.87 & 0.65 & 0.43 & 0.08 & 0.86\\
estimator 2, three initializations & 3 & 0.90 & 0.71 & 0.46 & 0.09 & 0.87\\
estimator 3, three initializations & 3 & 0.88 & 0.68 & 0.45 & 0.08 & 0.87\\
estimator 4, three initializations & 3 & 0.88 & 0.67 & 0.44 & 0.08 & 0.86\\}
\newcommand{\Nreserved}{4{,}659}
\newcommand{\Neligible}{13{,}397}

